Chameleon Cache: Approximating Fully Associative Caches with Random Replacement to Prevent Contention-Based Cache Attacks

Randomized, skewed caches (RSCs) such as CEASER-S have recently received much attention to defend against contention-based cache side channels. By randomizing and regularly changing the mapping(s) of addresses to cache sets, these techniques are designed to obfuscate the leakage of memory access patterns. However, new attack techniques, e.g., Prime+Prune+Probe, soon demonstrated the limits of RSCs as they allow attackers to more quickly learn which addresses contend in the cache and use this information to circumvent the randomization. To yet maintain side-channel resilience, RSCs must change the random mapping(s) more frequently with adverse effects on performance and implementation complexity. This work aims to make randomization-based approaches more robust to allow for reduced re-keying rates and presents Chameleon Cache. Chameleon Cache extends RSCs with a victim cache (VC) to decouple contention in the RSC from evictions observed by the user. The VC allows Chameleon Cache to make additional use of the multiple mappings RSCs provide to translate addresses to cache set indices: when a cache line is evicted from the RSC to the VC under one of its mappings, the VC automatically reinserts this evicted line back into the RSC by using a different mapping. As a result, the effects of previous RSC set contention are hidden and Chameleon Cache exhibits side-channel resistance and eviction patterns similar to fully associative caches with random replacement. We show that Chameleon Cache has performance overheads of < 1% and stress that VCs are more generically helpful to increase side-channel resistance and re-keying intervals of randomized caches.

==> Makefile <==
# Generic paper Makefile
#
# For usage hints, "make help"
#
#  To create a LaTeX diff against the hg "tip" revision, use the target
#  "diff" (or "viewdiff").
#  To use a revision other than "tip", speciff DIFF=x on the 
#  make command line to choose the revision x.
#

# Verbosity
ifeq (${V},1)
Q:=
else
Q:=@
endif

DOT_NATIVE = $(wildcard figures_native/*.dot)
DOT_PDF    = $(patsubst figures_native/%.dot,figures/%.pdf,$(DOT_NATIVE))

IPE_NATIVE = $(wildcard figures_native/*.ipe)
IPE_PDF    = $(patsubst figures_native/%.ipe,figures/%.pdf,$(IPE_NATIVE))

OO_NATIVE  = $(wildcard figures_native/*.odg)
OO_PDF     = $(patsubst figures_native/%.odg,figures/%.pdf,$(OO_NATIVE))

SVG_NATIVE  = $(wildcard figures_native/*.svg)
SVG_PDF     = $(patsubst figures_native/%.svg,figures/%.pdf,$(SVG_NATIVE))

TEX_NATIVE = $(wildcard figures_native/*.tex)
TEX_PDF    = $(patsubst figures_native/%.tex,figures/%.pdf,$(TEX_NATIVE))

PDF_NATIVE = $(wildcard figures_native/*.pdf)
PDF_PDF    = $(patsubst figures_native/%.pdf,figures/%.pdf,$(PDF_NATIVE))

.PHONY: all

BIBDIR     ?= /home/disy/lib/BibTeX:../../../bibtex:../bibtex
LaTeXEnv   = TEXINPUTS=".:/home/disy/lib/TeX:/home/disy/lib/ps:${TEXINPUTS}:"
BibTexEnv  = BIBINPUTS=".:${BIBDIR}:${BIBINPUTS}:"
BibFiles   = defs-abbrev,extra,combined,systems,fm,other

LaTeX      = ${LaTeXEnv} pdflatex -interaction=nonstopmode
LaTeXdiff  = ./tools/latexdiff
BibTeX     = ${BibTexEnv} bibtex
Fig2Eps    = fig2dev -L eps
Dia2Eps    = dia -t eps -e
AS         = $(shell which as)
CC         = $(shell which gcc)
GnuPlot	   = gnuplot
Inkscape   = $(shell which inkscape)
Eps2Pdf	   = epstopdf --outfile
PdfView	   = xpdf
Pdf2Ps	   = pdf2ps
RmCR       = tr -d '\r'
sed        = $(shell which sed)
#PdfView    = open -a preview
#PdfView    = acroread 
Lpr 	   = lpr
mv	   = mv
awk	   = awk
R	   = R

# Use either "report" or "paper", depending on the template.
# To add a further target, simply append the basename of the .tex file here
Targets    = chameleon_cache
SRCS = chameleon_cache.tex 


# CONFIGURATION OPTIONS
# =====================

# For ACM SIG camera ready submission. This will only work if Target
# is a single identifier. You should then be able to use the "camera" target,
# after setting CamRoot appropriately. Answer "no" for re-making references.bib
# Set CamRoot as the filename root per publisher's instructions.
# Should be <paperno>-<lastname-of-first-author>
CamRoot    = <paperno>-<last>
CamDir	   = cameraready

# Any other stuff that may be needed

# END CONFIGURATION OPTIONS
# =========================

Optional = $(addsuffix -diff, $(Targets))
All = $(Targets) $(Optional)
Diffopts= #--type=BWUNDERLINE #-c .latexdiffconfig --append-safecmd="Comment"

Gnuplot_Sources = $(wildcard figures/*.gnuplot)
Figures = $(Gnuplot_Sources:.gnuplot=.pdf)



Pdf = $(addsuffix .pdf, $(Targets))
Tex = $(addsuffix .tex, $(Targets))
Diff_Pdf = $(addsuffix .pdf, $(Optional))

.PHONY: FORCE

all: pdf
diff: diff_pdf
FORCE: pdf
ps: $(Ps)
pdf: $(Figures) Makefile $(Pdf)
diff_pdf: $(Figures) Makefile $(Diff_Pdf)

%.pdf: %.perf tools/bargraph.pl
	@echo $< '->' $@
	${Q} ${BarGraph} -pdf $< > $@

%.pdf: %.eps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.pdf: %.ps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

#%.eps: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -E $@ > /dev/null 2>&1

#%.pdf: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -A $@ > /dev/null 2>&1

# This target allows you to add figures which have the extension .c_pp that
# correspond to .c sources. Your .c sources can use the lines '/*<*/' and
# '/*>*/' to surround parts of the source you don't want shown in your PDF.
# This allows you to write a .c file that can be compile-checked here and then
# remove extraneous lines for display.
%.c_pp: %.c
	@echo $< '->' $@
	${Q}$(if ${CC},${CC} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.s_pp: %.s
	@echo $< '->' $@
	${Q}$(if ${AS},${AS} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.eps: %.dia
	@echo $< '->' $@
	${Q} ${Dia2Eps} $@ $<

%.eps: %.fig
	@echo $< '->' $@
	${Q} ${Fig2Eps} $< $@

%.eps: %.gnuplot
	@echo $< '->' $@
	${Q} ${GnuPlot} $<

%.eps: %.r
	@echo $< '->' $@
	${Q} ${R} --vanilla < $<

%.pdf: %.pdf-shipped
	cp $< $@

view: pdf
	${Q}for i in $(Pdf); do \
		$(PdfView) $$i & \
	done

viewdiff: diff
	${Q}for i in $(Diff_Pdf); do \
		$(PdfView) $$i & \
	done

print: pdf
	${Q}for i in $(Pdf); do \
		$(Lpr) $$i \
	done

clean:
	rm -f *.aux *.toc *.bbl *.blg *.dvi *.log *.pstex* *.eps *.cb *.brf \
		*.idx *.out *.ps *-diff.* *.mps .log *.diff chameleon_cache.pdf

help:
	@echo "Main targets: all diff camera view viewdiff print clean realclean tar"
	@echo "'make diff' will show changes to head revision"
	@echo "'make DIFF=<rev> diff' will show changes to revision <rev>"
	@echo "Avoid TeX \def with arguments, this breaks latexdiff (use \newcommand)"

figures/%.pdf: figures_native/%.dot
	dot -Tpdf -o $@ $<
	pdfcrop $@ $@-cropped
	mv $@-cropped $@

figures/%.pdf: figures_native/%.ipe
	ipetoipe -pdf $< $@

figures/%.pdf: figures_native/%.odg
	loffice --headless --convert-to pdf --outdir figures $<
	pdfcrop $@ $@-cropped
	mv $@-cropped $@

figures/%.pdf: figures_native/%.svg
	inkscape -z -D --file=$< --export-ignore-filters --export-pdf=$@

figures/%.pdf: figures_native/%.tex
	cd figures_native && ${PDFLATEX_CMD} -interaction=nonstopmode $(patsubst figures_native/%.tex,%.tex,$<)
	pdfcrop $(patsubst figures_native/%.tex,figures_native/%.pdf,$<) $@
	find figures_native -type f -iname "$(patsubst figures_native/%.tex,%,$<).*" ! -iname "*.tex" -delete

figures/%.pdf: figures_native/%.pdf
	pdfcrop $< $@

assets: $(DOT_PDF) $(IPE_PDF) $(OO_PDF) $(SVG_PDF) $(TEX_PDF) ${PDF_PDF}



##############################################################################

DIFF ?= tip

%-diff.dvi: %-diff.tex

%-diff.tex: %.tex FORCE
	@echo "====> Retrieving revision $(DIFF) of $<"
	hg cat -r $(DIFF) $<  > $(@:-diff.tex=-$(DIFF)-diff.tex)
	@echo "====> Creating diff of revision $(DIFF) of $<"
	$(LaTeXdiff) $(Diffopts) $(@:-diff.tex=-$(DIFF)-diff.tex) $< | \
	${RmCR} > $@

.PHONY: FORCE
FORCE:

# don't delete %.aux intermediates
.SECONDARY:

##############################################################################

Rerun = '(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)'
Rerun_Bib = 'No file.*\.bbl|Citation.*undefined'
Undefined = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
Error = '^! '


chameleon_cache.pdf: chameleon_cache.tex  $(Figures) Makefile ${SRCS}
	${Q}if ! test -e chameleon_cache.bbl || test chameleon_cache.bib -nt chameleon_cache.bbl; then rm -f chameleon_cache.bbl; fi
	@echo "====> LaTeX first pass: $(<)"
	${Q}$(LaTeX) $< >.log || if egrep -q $(Error) chameleon_cache.log ; then cat .log; rm $@; false ; fi
	${Q}if egrep -q $(Rerun_Bib) chameleon_cache.log ; then echo "====> BibTex" && ( $(BibTeX) chameleon_cache > .log || ( cat .log ; false ) ) && echo "====> LaTeX BibTeX pass" && $(LaTeX) >.log $< || if egrep -q $(Error) chameleon_cache.log ; then cat .log; rm $@; false ; fi ; fi
	${Q}if egrep -q $(Rerun) chameleon_cache.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) chameleon_cache.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) chameleon_cache.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if [ -a .NeedGS ]; then gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=tmp.pdf $@; mv tmp.pdf $@; fi
	@echo "====> Undefined references and citations in $(<):"
	@egrep -i $(Undefined) chameleon_cache.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" chameleon_cache.log || echo "None."

##############################################################################
# Generate a list of FIXMEs 
fixmes: 
	${Q}for i in $(Tex); do \
		echo "FIXMEs in $$i:"; \
		nl -b a $$i | grep "FIXME{" | nl -b a; \
		echo -n "Total FIXMES: " && grep "FIXME{" $$i | wc -l; \
		echo; \
	done


